Mutual or Unrequited Love: Identifying Stable Clusters in Social Networks with Uni- and Bi-directional Links

Many social networks, e.g., Slashdot and Twitter, can be represented as directed graphs (digraphs) with two types of links between entities: mutual (bi-directional) and one-way (uni-directional) connections. Social science theories reveal that mutual connections are more stable than one-way connections, and one-way connections exhibit various tendencies to become mutual connections. It is therefore important to take such tendencies into account when performing clustering of social networks with both mutual and one-way connections. In this paper, we utilize the dyadic methods to analyze social networks, and develop a generalized mutuality tendency theory to capture the tendencies of those node pairs which tend to establish mutual connections more frequently than those occur by chance. Using these results, we develop a mutuality-tendency-aware spectral clustering algorithm to identify more stable clusters by maximizing the within-cluster mutuality tendency and minimizing the cross-cluster mutuality tendency. Extensive simulation results on synthetic datasets as well as real online social network datasets such as Slashdot, demonstrate that our proposed mutuality-tendency-aware spectral clustering algorithm extracts more stable social community structures than traditional spectral clustering methods.

==> ICDCS2012_2_related.tex <==
%\section{Related Work}\label{sec:related}
\noindent{\textbf{Related Work}.} Studying the social network structure and properties of social ties
have been an active topic
recently~\cite{kurucz2007spectral,smyth2005spectral,mishra2007clustering}.
Due to the space limitation, we only briefly discuss a few related
works that are directly related to our study here.

\noindent\textbf{Dyads analysis.} Social scientists have observed
that mutual
social relations and one-way relations in social networks
exhibit different stabilities, i.e., mutual relations are more stable
than one-way relations~\cite{wolfe1997social}. To measure the tendencies
of node pairs to establish mutual relations than those occur by chance, Katz
and Powell~\cite{katz1955measurement} produce the mutuality tendency. Moreover,
recent papers~\cite{kwak2011fragile,jamali2011modeling} reveal and confirm by
empirical studies that the mutual social connections are more stable relations than one-way relations.

\noindent\textbf{Spectral clustering.} The graph spectral clustering
problem has been studied
extensively~\cite{Luxburg:2007,pami:ShiM00,WangD:KDD10,icmlZhouHS05,
WestonLIZEN05}. Most of them focus on the undirected graphs,
e.g.,~\cite{Luxburg:2007,pami:ShiM00,WangD:KDD10}, while

a few
algorithms are designed for directed graphs. For examples, Zhou and
et al~\cite{icmlZhouHS05, WestonLIZEN05} apply the spectral
clustering to symmetrized random walk flow matrix, where the
minimized cut function is then the total random walk flow across
clusters. In ~\cite{edbt:SatuluriP11}, several symmetrization
methods are discussed, including the symmetrized adjacency matrix
$\bar{A}=(A+A^T)/{2}$, The bibliographic coupling matrix $AA^T$ and
the co-citation strength matrix $A^TA$, etc.

Moreover, some other generalizations of the spectral clustering
methods are also introduced, e.g.,~\cite{kunegis:signed-kernels}
proposes signed Laplacian matrix as objective for clustering in
signed networks, where positive and negative links, for example,
interpreted as trust and distrust relations, are jointly considered
while performing the clustering. In a more general setting,
~\cite{2006ICMLmultirelation} studies the spectral clustering
algorithm for multi-relation networks, where entities in a network
are connected with multiple types of relations. The authors in~\cite{smyth2005spectral}
develop spectral clustering algorithms to realize modularity matrix based community detection.

In our paper, we focus on directed graph spectral clustering, aiming
to detect stable clusters by considering the tendencies of node pairs to establish
mutual connections, namely, nodes with more tendencies to get mutually connected
are grouped together, whereas those with one-way (unstable) connections are more likely
to be placed in different clusters.

